Dynamical intricacy and average sample complexity

We propose a new way to measure the balance between freedom and coherence in a dynamical system and a new measure of its internal variability. Based on the concept of entropy and ideas from neuroscience and information theory, we define \emph{intricacy} and \emph{average sample complexity} for topological and measure-preserving dynamical systems. We establish basic properties of these quantities, show that their suprema over covers or partitions equal the ordinary entropies, compute them for many shifts of finite type, and indicate natural directions for further research.

==> 2lettersft_Asqpostable.tex <==
\begin{center}
\begin{longtable}{@{}m{.04\textwidth}m{.15\textwidth}m{.05\textwidth}m{.25\textwidth}m{.08\textwidth}m{.12\textwidth}m{.12\textwidth}@{}}
\toprule
SFT& \hspace{.4in}$M$ & $\rho(M)$
   &\ \hspace{.45in} \text{Graph} & \text{Entropy} & $\Asc(X,\sigma)$ & $\Int(X,\sigma)$
   \\
   \midrule
   
   \endfirsthead
   \multicolumn{7}{l}{{Continued from previous page}}\\
   \toprule
SFT& \hspace{.4in}$M$ & $\rho(M)$
   &\ \hspace{.45in} \text{Graph} & \text{Entropy}  & $\Asc(X,\sigma)$ & $\Int(X,\sigma)$
   \\
   \midrule
   
   \endhead
   
   \bottomrule
  \multicolumn{7}{r}{{Continued on next page}}
   \endfoot
   \bottomrule
   \endlastfoot

 2 & $\left(
\begin{array}{cc}
 1 & 1 \\
 1 & 0 \\
\end{array}
\right)$ & 2 &   \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjGMS}& 0.481 & 0.286 & 0.091 \\
 3 & $\left(
\begin{array}{cc}
 1 & 1 \\
 1 & 1 \\
\end{array}
\right) $& 1 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjF2}  & 0.693 & 0.347 & 0 \\

\end{longtable}
\end{center}

==> 3lettersft_Asqpostable.tex <==
\begin{center}
\begin{longtable}{@{}m{.04\textwidth}m{.15\textwidth}m{.05\textwidth}m{.25\textwidth}m{.08\textwidth}m{.12\textwidth}m{.12\textwidth}@{}}
\toprule
SFT& \hspace{.4in}$M$ & $\rho(M)$
   &\ \hspace{.45in} \text{Graph} & \text{Entropy} & $\Asc(X,\sigma)$ & $\Int(X,\sigma)$
   \\
   \midrule
   
   \endfirsthead
   \multicolumn{7}{l}{{Continued from previous page}}\\
   \toprule
SFT& \hspace{.4in}$M$ & $\rho(M)$
   &\ \hspace{.45in} \text{Graph} & \text{Entropy}  & $\Asc(X,\sigma)$ & $\Int(X,\sigma)$
   \\
   \midrule
   
   \endhead
   
   \bottomrule
  \multicolumn{7}{r}{{Continued on next page}}
   \endfoot
   \bottomrule
   \endlastfoot
   
 4 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA4}& 0.693 & 0.448 & 0.203 \\
 5 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 &\includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA5}  & 0.693 & 0.448 & 0.203  \\
 6 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA6}& 0.881 & 0.491 & 0.101 \\
 7 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 &\includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA7}  & 1.010 & 0.523 & 0.036 \\
 14 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ & 2 &\includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA14}  & 0.693 & 0.448 & 0.203 \\
 15 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA15} & 0.693 & 0.448 & 0.203 \\
 16 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ & 2 &\includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA16}  & 0.844 & 0.485 & 0.126 \\
 20 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 &\includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA20}  & 0.810 & 0.483 & 0.156 \\
 21 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 &\includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA21}  & 0.764 & 0.457 & 0.150 \\
 22 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA22} & 0.881 & 0.491 & 0.101 \\
 23 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA23} & 0.881 & 0.491 & 0.101 \\
 24 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA24} & 0.962 & 0.518 & 0.074 \\
 26 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA26} & 0.693 & 0.430 & 0.167 \\
 28 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 &\includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA28}  & 0.810 & 0.464 & 0.118 \\
 29 &$ \left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA29} & 0.881 & 0.491 & 0.101 \\
\end{longtable}
\end{center}

==> 5stringscomptable.tex <==

\begin{table}[h]
\centering
\begin{tabular}{@{}m{.1\textwidth}m{.1\textwidth}@{}}
\toprule

 $w$& $\Asw(w)$\\
      \midrule
 11111 & 1.00 \\
 00000 & 1.00 \\
 11110 & 1.75625 \\
 10101 & 1.75625 \\
 10000 & 1.75625 \\
 01111 & 1.75625 \\
 01010 & 1.75625 \\
 00001 & 1.75625 \\
 11100 & 1.9375 \\
 11000 & 1.9375 \\
 00111 & 1.9375 \\
 00011 & 1.9375 \\
 11101 & 1.9875 \\
 10111 & 1.9875 \\
 01000 & 1.9875 \\
 00010 & 1.9875 \\

 \bottomrule
\end{tabular}
\qquad
\begin{tabular}{@{}m{.1\textwidth}m{.1\textwidth}@{}}
\toprule

 $w$& $\Asw(w)$\\
      \midrule
 11011 & 2.03125 \\
 00100 & 2.03125 \\
 11010 & 2.05625 \\
 10110 & 2.05625 \\
 10100 & 2.05625 \\
 10010 & 2.05625 \\
 10001 & 2.05625 \\
 01110 & 2.05625 \\
 01101 & 2.05625 \\
 01011 & 2.05625 \\
 01001 & 2.05625 \\
 00101 & 2.05625 \\
 11001 & 2.15 \\
 10011 & 2.15 \\
 01100 & 2.15 \\
 00110 & 2.15 \\
  \bottomrule
\end{tabular}
\caption{Complexity of all strings of $0$s and $1$s of length $5$.\label{seq4comp}}
\end{table}

==> all2lettersfttable.tex <==

\begin{center}
\begin{longtable}{@{}m{.05\textwidth}m{.15\textwidth}m{.05\textwidth}m{.25\textwidth}m{.08\textwidth}m{.08\textwidth}m{.08\textwidth}m{.08\textwidth}@{}}
\toprule
SFT& \hspace{.3in}$M$ & $\rho(M)$
   &\ \hspace{.45in} \text{Graph} & \text{Entropy} & $H(10)$ & $\Asc(10)$ & $\Int(10)$
   \\
   \midrule
   
   \endfirsthead
   \multicolumn{8}{l}{{Continued from previous page}}\\
   \toprule
SFT&\hspace{.4in}$M$&$\rho(M) $
   & \ \hspace{.45in} \text{Graph}  & \text{Entropy} & $H(10)$ & $\Asc(10)$ & $\Int(10)$
   \\
   \midrule
   
   \endhead
   
   \bottomrule
  \multicolumn{8}{r}{{Continued on next page}}
   \endfoot
   \bottomrule
   \endlastfoot
   

 1 & $\displaystyle\left(
\begin{array}{cc}
0&1\\
1&0\\
\end{array}
\right)$ & $\infty$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/Adjper2} & 0.000 & 0.069 & 0.069 & 0.069 \\ \\
 2 & $\left(
\begin{array}{cc}
 1 & 1 \\
 1 & 0 \\
\end{array}
\right)$& 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjGMS}  & 0.481 & 0.497 & 0.291 & 0.085 \\ \\
 3 & $\left(
\begin{array}{cc}
 1 & 1 \\
 1 & 1 \\
\end{array}
\right)$ & 1 &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjF2} & 0.693 & 0.693 & 0.347 & 0.000 \\


\end{longtable}
\end{center}


==> all3lettersftneuraltable.tex <==
\begin{center}
\begin{longtable}{@{}m{.08\textwidth}m{.15\textwidth}m{.25\textwidth}m{.08\textwidth}m{.08\textwidth}m{.08\textwidth}m{.08\textwidth}@{}}
\toprule
SFT& \hspace{.4in}$M$   &\ \hspace{.45in} \text{Graph} & \text{Entropy} & $H(10)$ & $\Asc(10)$ & $\Int(10)$
   \\
   \midrule
   
   \endfirsthead
   \multicolumn{7}{l}{{Continued from previous page}}\\
   \toprule
SFT&\hspace{.4in}$M$   & \ \hspace{.45in} \text{Graph}  & \text{Entropy} & $H(10)$ & $\Asc(10)$ & $\Int(10)$
   \\
   \midrule
   
   \endhead
   
   \bottomrule
  \multicolumn{7}{r}{{Continued on next page}}
   \endfoot
   \bottomrule
   \endlastfoot


 1 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA1} & 0.000 & 0.110 & 0.100 & 0.090 \\
 2 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA2} & 0.382 & 0.448 & 0.304 & 0.16 \\
 3 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA3} & 0.562 & 0.614 & 0.38 & 0.146 \\
 4 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA4} & 0.693 & 0.734 & 0.428 & 0.122 \\
 5 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA5} & 0.693 & 0.734 & 0.428 & 0.122 \\
 6 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA6} & 0.881 & 0.9 & 0.481 & 0.062 \\
 7 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA7} & 1.005 & 1.013 & 0.519 & 0.026 \\
 8 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA8} & 1.099 & 1.099 & 0.549 & 0. \\
 9 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA9} & 0.281 & 0.361 & 0.26 & 0.159 \\
 10 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA10} & 0.609 & 0.648 & 0.382 & 0.115 \\
 11 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA11} & 0.609 & 0.648 & 0.382 & 0.115 \\
 12 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA12} & 0.791 & 0.811 & 0.443 & 0.074 \\
 13 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA13} & 0.481 & 0.545 & 0.357 & 0.169 \\
 14 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA14} & 0.693 & 0.734 & 0.428 & 0.122 \\
 15 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA15} & 0.693 & 0.734 & 0.428 & 0.122 \\
 16 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA16} & 0.844 & 0.867 & 0.472 & 0.077 \\
 17 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA17} & 0.481 & 0.545 & 0.342 & 0.14 \\
 18 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA18} & 0.693 & 0.734 & 0.42 & 0.106 \\
 19 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA19} & 0.693 & 0.734 & 0.42 & 0.106 \\
 20 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA20} & 0.81 & 0.844 & 0.467 & 0.091 \\
 21 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA21} & 0.764 & 0.792 & 0.443 & 0.093 \\
 22 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA22} & 0.881 & 0.9 & 0.481 & 0.062 \\
 23 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA23} & 0.881 & 0.9 & 0.481 & 0.062 \\
 24 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA24} & 0.962 & 0.978 & 0.51 & 0.043 \\
 25 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA25} & 0.347 & 0.416 & 0.245 & 0.075 \\
 26 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA26} & 0.693 & 0.722 & 0.414 & 0.106 \\
 27 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA27} & 0.589 & 0.631 & 0.373 & 0.115 \\
 28 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA28} & 0.81 & 0.83 & 0.453 & 0.076 \\
 29 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 1 \\
\end{array}
\right)$ &  \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA29} & 0.881 & 0.9 & 0.481 & 0.062 \\   

\end{longtable}
\end{center}

==> all3lettersfttable.tex <==
\begin{center}
\begin{longtable}{@{}m{.04\textwidth}m{.15\textwidth}m{.05\textwidth}m{.25\textwidth}m{.08\textwidth}m{.08\textwidth}m{.08\textwidth}m{.08\textwidth}@{}}
\toprule
SFT& \hspace{.35in}$M$ & $\rho(M)$
   &\ \hspace{.45in} \text{Graph} & \text{Entropy} & $H(10)$ & $\Asc(10)$ & $\Int(10)$
   \\
   \midrule
   
   \endfirsthead
   \multicolumn{8}{l}{{Continued from previous page}}\\
   \toprule
SFT&\hspace{.35in}$M$&$\rho(M) $
   & \ \hspace{.45in} \text{Graph}  & \text{Entropy} & $H(10)$ & $\Asc(10)$ & $\Int(10)$
   \\
   \midrule
   
   \endhead
   
   \bottomrule
  \multicolumn{8}{r}{{Continued on next page}}
   \endfoot
   \bottomrule
   \endlastfoot
   
 1 &$\displaystyle \left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right) $& $\infty$ & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA1}&0.000 & $0.110$ & 0.110 & 0.110 \\
 2 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 4 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA2}&0.382 & 0.448 & 0.342 & 0.236 \\
 3 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 3 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA3}&0.562 & 0.614 & 0.416 & 0.218 \\
 4 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA4}&0.693 & 0.734 & 0.458 & 0.182 \\
 5 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA5}& 0.693 & 0.734 & 0.458 & 0.182 \\
 6 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA6}& 0.881 & 0.900 & 0.496 & 0.093 \\
 7 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA7}& 1.010 & 1.010 & 0.526 & 0.039 \\
 8 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ & 1 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA8}& 1.100 & 1.100 & 0.549 & 0.000 \\
 9 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 5 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA9}& 0.281 & 0.361 & 0.297 & 0.234 \\
 10 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ & 3 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA10}& 0.609 & 0.648 & 0.409 & 0.171 \\
 11 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 3 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA11}&  0.609 & 0.648 & 0.409 & 0.171 \\
 12 & $\left(
\begin{array}{ccc}
 0 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ & 3 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA12}&  0.791 & 0.811 & 0.460 & 0.110 \\
 13 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 3 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA13}&  0.481 & 0.545 & 0.399 & 0.254 \\
 14 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 0 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA14}& 0.693 & 0.734 & 0.458 & 0.182 \\
 15 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA15}& 0.693 & 0.734 & 0.458 & 0.182 \\
 16 & $\left(
\begin{array}{ccc}
 1 & 1 & 0 \\
 0 & 1 & 1 \\
 1 & 1 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA16}& 0.844 & 0.867 & 0.491 & 0.115 \\
 17 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 4 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA17}&0.481 & 0.545 & 0.377 & 0.208 \\
 18 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 3 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA18}& 0.693 & 0.734 & 0.446 & 0.158 \\
 19 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 3 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA19}& 0.693 & 0.734 & 0.446 & 0.158 \\
 20 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA20}& 0.810 & 0.844 & 0.490 & 0.136 \\
 21 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA21}& 0.764 & 0.792 & 0.466 & 0.140 \\
 22 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA22}&  0.881 & 0.900 & 0.496 & 0.093 \\
 23 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA23}&0.881 & 0.900 & 0.496 & 0.093 \\
 24 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 1 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA24}&0.962 & 0.978 & 0.521 & 0.064 \\
 25 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 0 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & $\infty$ & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA25}& 0.347 & 0.416 & 0.256 & 0.096 \\
 26 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 0 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA26}& 0.693 & 0.722 & 0.440 & 0.158 \\
 27 & $\left(
\begin{array}{ccc}
 0 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 4 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA27}&0.589 & 0.631 & 0.400 & 0.170 \\
 28 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 0 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA28}& 0.810 & 0.830 & 0.472 & 0.114 \\
 29 & $\left(
\begin{array}{ccc}
 1 & 1 & 1 \\
 1 & 1 & 0 \\
 1 & 0 & 1 \\
\end{array}
\right)$ & 2 & \includegraphics[width=1.5in,keepaspectratio]{Dissertation_Images/AdjA29}& 0.881 & 0.900 & 0.496 & 0.093 \\

\end{longtable}
\end{center}

